Equivariant Point Network for 3D Point Cloud Analysis

Features that are equivariant to a larger group of symmetries have been shown to be more discriminative and powerful in recent studies. However, higher-order equivariant features often come with an exponentially-growing computational cost. Furthermore, it remains relatively less explored how rotation-equivariant features can be leveraged to tackle 3D shape alignment tasks. While many past approaches have been based on either non-equivariant or invariant descriptors to align 3D shapes, we argue that such tasks may benefit greatly from an equivariant framework. In this paper, we propose an effective and practical SE(3) (3D translation and rotation) equivariant network for point cloud analysis that addresses both problems. First, we present SE(3) separable point convolution, a novel framework that breaks down the 6D convolution into two separable convolutional operators alternatively performed in the 3D Euclidean and SO(3) spaces. This significantly reduces the computational cost without compromising the performance. Second, we introduce an attention layer to effectively harness the expressiveness of the equivariant features. While jointly trained with the network, the attention layer implicitly derives the intrinsic local frame in the feature space and generates attention vectors that can be integrated into different alignment tasks. We evaluate our approach through extensive studies and visual interpretations. The empirical results demonstrate that our proposed model outperforms strong baselines in a variety of benchmarks

==> figures/fig_attention_pool.tex <==
\begin{figure*}[t]
 \begin{center}
  \centering
  \includegraphics[width=0.8\linewidth]{attention_pool.pdf}
 \end{center}
 \caption{Our proposed \poolingName{} layer consumes permuted features, which is the output of our equivariant point network (\modelNameShort{}) given rotated point cloud, and aggregate them into invariant feature in a weighted sum manner. }{}
 \label{fig:pool}
\end{figure*}

==> figures/fig_example.tex <==
\begin{figure}[htb]
 \begin{center}
  \centering
  \includegraphics[width=1\linewidth]{plholder.png}
 \end{center}
 \Caption{Network Architecture.}{}
 \label{fig:archi}
\end{figure}

==> figures/fig_network_architecture.tex <==
\begin{figure}[t]
 \begin{center}
  \centering
  \includegraphics[width=1\linewidth]{network_architecture.pdf}
 \end{center}
 \caption{Our proposed architecture. (a) Given an input point cloud, we first lift it to feature space (b) where the appended initial features set as one. (c) Each data is then passed through a sequence of \convNameShort{} to obtain \seThree{} equivariant features. (d) We mean pool the feature spatially and (e) the resulting \soThree{} equivariant features are used as input to our \poolingName{} layer. The final output is thus a \seThree{} invariant feature.}{}
 \label{fig:pipeline}
\end{figure}

==> figures/fig_res_modelnet_ablation.tex <==
\begin{figure}[t]
 \begin{center}
  \centering
  \includegraphics[width=1.0\linewidth]{tsne_cls}
 \end{center}
 \caption{t-SNE embeddings of the equivariant features of 200 airplanes 3D shapes, learnt by different pooling methods. Each datapoint, drawn as circle, is a feature of a single airplane instance defined at rotation group $\soAnc \in \SoAncGroup$. The circles are colored by their associated rotation. The sharp contrast in clustering behaviors are very indicative of how choice of pooling method affects group structures in learned features. }
% \vspace{-10pt}
 \label{fig:pool_tsne}
\end{figure}

==> figures/fig_teaser2.tex <==
\begin{figure}[t]
 \begin{center}
  \centering
  \includegraphics[width=0.3\linewidth]{placeholder.pdf}
 \end{center}
 \caption{\Note{We propose \convNameShort{}, a convolution operator on point clouds that takes either scalar or spherical features as input and output convolved spherical features on each sample points that are rotation-equivariant to the input. \convNameShort{} is able to effectively aggregate rotation- and translation-agnostic features for dense point could matching problem.} }{}
 \label{fig:teaser2}
\end{figure}

==> hackbibstyle.tex <==
\setlength{\topsep}{0ex}
\setlength{\itemsep}{0ex}
\setlength{\partopsep}{0ex}
\setlength{\parsep}{0ex}
\setlength{\parskip}{1ex}
%\footnotesize


==> note.tex <==
\section{Note}
\label{sec:note}


This is note section!
\begin{description}
	\item[Oct. 19, 2019]
	{
		
		\haiwei{I'm good!} %haiwei
		
		\shichen{I'm good!} %shichen
		
		\weikai{I'm good!} %weikai
	}
\end{description}


==> sections/implementation.tex <==
\section{Implementation}
\label{sec:imp}

==> sections/loss.tex <==
\subsection{Triplet Loss for Feature Matching}
\label{sec:loss}

For feature matching, we designed a variation of the hardest-in-batch triplet loss inspired by \cite{hermans2017defense} and \cite{gojcic2019perfect}:

\begin{align*} 
	\loss_{BH}(\batch, \rotation) = \frac{1}{\batch}\sum^{\lvert\batch\rvert}_{i=1} \text{max}(0, \lvert\lvert \sphFeat(\batch^a_i) -  \rotation\sphFeat(\batch^p_i) \rvert \rvert_2 \\
		- \underset{{\substack{\text{j}=1\ldots\lvert\batch\rvert\\ \text{j}\neq\text{i}}}}{\text{min}} \lvert\lvert \sphFeat(\batch^a_i) -  \rotation\sphFeat(\batch^p_j) \rvert \rvert_2 + m )
\end{align*}

Similar to \cite{gojcic2019perfect}, the loss is defined for a mini-batch $\batch$ in training, and $\batch^a$, $\batch^p$ represent the anchor and positive input samples. The hardest non-corresponding samples in the mini-batch are utilized as the negative samples. $m$ is the margin between the positive and the negative pairs. The extra component of this loss function is the inclusion of a known rotation $\rotation$. When the feature $\sphFeat$ is equivariant to rotation, $\rotation$ is used to transform the positive samples to align with the anchors, such that the loss encourages the network to learn canonical shape information. When the feature $\sphFeat$ is invariant, $\rotation$ is simply the identity transformation.

==> sections/method_conv.tex <==
\subsection{Point Cloud Convolution with Conic Filters}
\label{sec:conv}

\shichen{
  our conv:
  \begin{itemize}
    \item similar to kpconv: directly apply on points, points as kernel, natural point cloud conv definition.
    \item use explicit kernel that could be more expressive than implicit kernel(e.g. pointnet)
    \item use polar-coordinate to locate kernels in the cone, learn meaningful features
  \end{itemize}
}


\paragraph{Spherical Point Convolution}
\shichen{Rename the operator}

\input{figures/fig_conic_conv}

\haiwei{
	The key element of Spherical Point CNN is the Spherical Point Convolution that operates on a set of spherical points $\{\sphpoint_i\}$. 
	(or say that the domain it operates on is group of spherical signals with coordinates centers ($\Point\times\sphere\rightarrow\mathbb{R}^{\sphFeatDim}$, which in implementation is discretized into the space $\mathbb{R}^{\sphFeatNum\times\sphFeatAnc\times\sphFeatDim}$ with $\sphFeatAnc$ anchor directions).  
}

Previous works study the general definition of a point convolution (cite: pointnet, pointnet++, kpconv...), we formulate our \convNameFull{} by expanding this operation to the field of spherical features inspired from the continuous form of spherical convolution function (equ~\ref{cont_sph_conv}). 
Specifically, we discretize the spherical feature with a uniformly parametrization of $\sphFeatAnc$ points, such that $\SphFeat \in \mathbb{R}^{\sphFeatNum\times\sphFeatAnc\times\sphFeatDim}$. 
We denote each point on the parameterized sphere as an anchor direction.
The proposed \convNameShort{} takes spherical features $\SphFeat$ with $\sphFeatDimIn$ dimensions as input and outputs spherical features with $\sphFeatDimOut$ dimensions, which is defined on a point $\point$ and anchor direction $\coneDirec$ as:

\begin{equation} \label{spconv}
  (\SphFeat \ast \kernelFunc)(\point, \coneDirec) = \sum_{\point_i \in \neighbor_{\point, \coneDirec}} \kernelFunc(\point_i - \point, \coneDirec)\sphFeat_{i, \coneDirec},
\end{equation}

\noindent where the neighbor points are chosen based on both their spatial and angular distance to the center point $\point$ and direction $\coneDirec$, which is given by $\neighbor_{\point, \coneDirec} = \left\{ \point_i \in \Point\ \big|\ \lVert \point_i - \point \rVert \leqslant \coneR \wedge \langle\point_i -\point, \coneDirec\rangle \leqslant \frac{\coneAngle}{2} \right\}$.
 $\kernelFunc$ is our proposed \convNameFull{} kernel defined in the shape of a cone with its angle set as $\coneAngle$ and its axis rotated to $\coneDirec$.
Since $\kernelFunc$ is circular symmetry, the rotation of its axis is reduced to $\sphere$ and its kernels are in the shape of \textit{circles}.

Similar to (cite: kpconv, pointconv, etc.), we define our convolution with \textit{explicit kernel circles} uniformly distributed in the cone.
For kernel size of $\kernelNum$, each kernel could be expressed as its angle to the north pole ($\coneDirec$) and its distance to origin $\kernelPos_k = (\kernelAng_k, \kernelDis_k)$.
We believe such design enhances the expressiveness of the networks.

The convolution is computed as a summation of coefficient of each neighbor points and each kernel circles, which could help the network learn meaningful rotation-equivariant features.
Therefore, the kernel function at point $\point_i - \point$ is,

\begin{equation}
  \kernelFunc(\point_i - \point, \coneDirec) = \sum_{k \leqslant \kernelNum}\kernelCoeff(\neighborPos_i,\kernelPos_k)\kernelWeight_k,
%  \kernelFunc(\neighborPos_i, \coneDirec) = \sum_{k \leqslant \kernelNum}\kernelCoeff(\langle\neighborPos_i, \coneDirec\rangle, \lVert\pointDiff_i\rVert, \kernelPos_k)\kernelWeight_k,
\end{equation}

\noindent where $\neighborPos_i = (\langle\point_i - \point, \coneDirec\rangle, \lVert\point_i - \point\rVert)$ is the in-plane polar coordinate of $\point_i - \point$, and $\kernelCoeff(\cdot, \cdot)$ is a coefficient kernel function between two points (e.g. gaussian kernel, linear kernel, etc.).

We prove that the proposed \convNameFull{} is 1) rotation equivariance; 2) translation equivariance.

Theorem 1: The proposed convolution operator is rotation equivariance w.r.t. rotation $\rotation$:
\begin{equation}
  \rotation(\convFunc)(\point, \coneDirec) = (\rotation\SphFeat \ast \kernelFunc)(\point, \coneDirec)
\end{equation}

\begin{align*}
  \rotation(\SphFeat \ast \kernelFunc)(\point, \coneDirec) &= (\SphFeat \ast \kernelFunc)(\rotation\point, \rotation\coneDirec)\\
  &= \sum_{k \leqslant K}\kernelCoeff(\langle\rotation\pointDiff_i, \rotation\coneDirec\rangle, \lVert\rotation\pointDiff_i\rVert, \kernelPos_k)\kernelWeight_k \sphFeat_{\rotation i, \rotation\coneDirec}\\
  &= \sum_{k \leqslant K}\kernelCoeff(\langle\pointDiff_i, \coneDirec\rangle, \lVert\pointDiff_i\rVert, \kernelPos_k)\kernelWeight_k \sphFeat_{\rotation i, \rotation\coneDirec}\\
  &= (\rotation\SphFeat \ast \kernelFunc)(\point, \coneDirec)
\end{align*}

Theorem 2: The proposed convolution operator is translation equivariance w.r.t. translation $\translation$:
\begin{equation}
  \translation(\convFunc)(\point, \coneDirec) = (\translation\SphFeat \ast \kernelFunc)(\point, \coneDirec)
\end{equation}

\begin{align*}
  \translation(\SphFeat \ast \kernelFunc)(\point, \coneDirec) &= (\SphFeat \ast \kernelFunc)(\translation\point, \coneDirec)\\
  &= \sum_{k \leqslant K}\kernelCoeff(\langle\translation\pointDiff_i, \coneDirec\rangle, \lVert\translation\pointDiff_i\rVert, \kernelPos_k)\kernelWeight_k \sphFeat_{\translation i, \coneDirec}\\
  &= \sum_{k \leqslant K}\kernelCoeff(\langle\pointDiff_i, \coneDirec\rangle, \lVert\pointDiff_i\rVert, \kernelPos_k)\kernelWeight_k \sphFeat_{\translation i, \coneDirec}\\
  &= (\translation\SphFeat \ast \kernelFunc)(\point, \coneDirec)
\end{align*}



\paragraph{Spherical Convolution}

Key to translation Equivariance

==> sections/method_equiv.tex <==
\subsection{Equivariant Network Layer}
\label{sec:equiv_layer}

\input{figures/fig_network_architecture}

Inspired by previous designs of point set CNN, we have designed SE(3) equivariant network layers that accommodate input in the form of 3D point clouds. This section will detail the important layers that require special care to preserve rotational information. 

\paragraph{Grouping Layer}

In the absence of a regular grid structure, points in a point cloud are usually grouped into local neighborhoods through radius search or KNN. Points in a neighborhood are usually subsampled to a fixed amount. Since point cloud can display varying densities, ball query is a more preferable subsampling strategy, as it restricts subsampled points to a fixed area. When points are sparser than required in a local region, either the remaining points are resampled from the already selected points, or \textit{shadow points}, dummy nodes that are expected to have no influence on the weight computations, are inserted to fill the remaining gap. (note: shadow points is a term coined in KPConv) 

In our network, local neighborhoods corresponding to the receptive field of the filter are \textbf{conic regions} of a $r$-radius ball, as opposed to balls of points in many previous architectures. A conic region, as introduced in section (?), is parameterized by an aperture $\coneAngle$ and a viewing direction $\coneDirec$

 We therefore choose a grouping strategy that first use ball query to group points into $\groupdim$ balls, whose centroids are points selected by the furthest point sampling algorithm. Then, points in each $r$-radius ball are further grouped into $\sphFeatAnc$ conic regions, whose viewing directions are the anchor directions. Each conic region selects $\anndim$ points that falls into its field of view (based on Equation ?), including the centroid of the ball. When less than $\anndim$ points are available, the remaining points are filled with shadow points. (shall we talk about why kernel point influences are not normalized. Repetitive sampling has a negative impact on unnormalized influences, while shadow points does not.) 
 
\paragraph{Spherical Point Convolution Layer}

In translation-equivariant CNN, the effective receptive field (cite someone?) of a neuron can be increased in deeper layer, given a kernel size that is larger than 1x1. Spherical Point Convolution formulated by Eq.\ref{spconv} aggregates information along the convex cone emanated from the conic kernel. It is worth noting that $\sphFeat_{i, \coneDirec}$ in  Eq.\ref{spconv} only maintains feature at one direction before multiplying with the kernel functions. The receptive field of a kernel at anchor $\anchor_i$ thus extends further along its viewing direction in deeper layer, but may be limited in learning from features in other directions of the visible spherical points. 
To circumvent such limitation, we employ a slightly altered spherical point convolution of the form:

\begin{equation} \label{intraconv}
  (\SphFeat \ast \kernelFunc)(\point) = \sum_{m \leq \sphFeatAnc} \kernelFunc(\kernelAng_m)\sphFeat_{\coneDirec_m},
\end{equation} 

We term the above convolution Spherical Anchor Convolution, as the convolution aggregates information across features across anchors in the same sphere. The convolution can be proved equivariant to $SE(3)$ similar to Eq.? 

\paragraph{Interpolation of Spherical Feature}

 \convNameShort{} discretizes spherical features by a uniformly sampled set of anchor directions. Both rotation of the feature and resampling on the sphere amounts to interpolating the features at new directions of the anchors. Thus, similar to \cite{qi2017pointnet++}, we adopt a propagation strategy based on a nearest-point interpolation method, with a spherical gaussian interpolant:

\begin{align*} \label{propagation}
  \sphFeat(\point, \coneDirec) &= \frac{\sum_{\coneDirec_i \in \neighbor_\coneDirec} \kernelCoeff(\coneDirec,\coneDirec_i)\sphFeat(\point,\coneDirec_i)}{\sum_{\coneDirec_i \in \neighbor_\coneDirec} \kernelCoeff(\coneDirec,\coneDirec_i) } \\
  \\
  \mbox{where} \;\;\; \kernelCoeff(\coneDirec,\coneDirec_i) &= e^{\lambda  (\langle \coneDirec,\coneDirec_i\rangle - 1)}
\end{align*}



\paragraph{Pooling Layer}

Pooling operation 



==> sections/method_prelim.tex <==
\subsection{Preliminaries}
\label{sec:prelim}

\paragraph{Representation}

A unit 2-sphere $\sphere$ is defined as the set of points $\{(x,y,z)|x^2+y^2+z^2=1\}$ in $\mathbb{R}^3$. 

In this paper, we consider a convex conic region emanating from the origin of a 2-sphere to be a convex spherical sector parameterized by its cone angle $\coneAngle$ (or aperture) and its radius $\coneR$. Additionally, each conic region considered in this paper is given a viewing direction $\coneDirec \in \sphere$ as its axis. The set of points in the conic region is therefore ...


A point convolution can be modeled by the convolution of point features from $\SphFeat \in \mathbb{R}^{\sphFeatNum \times \sphFeatDim}$ and a kernel function $\kernelFunc$ on points $\point_i$ from a point set $\Point \in \mathbb{R}^{\sphFeatNum \times 3}$ in 3D:

\begin{equation} \label{pcconv}
  (\convFunc)(\point) = \sum_{\point_i \in \neighbor_\point} f(\point_i) \kernelFunc(\point_i - \point)
\end{equation} 


Spherical feature $\SphFeat : \sphere \rightarrow \mathbb{R}^\sphFeatDim$. \shichen{don't understand} \haiwei{maybe rename to spherical feature or spherical signal}

Spherical point: given a point set $\Point \in \mathbb{R} ^{\sphFeatNum \times 3}$, spherical points $\{\sphpoint_i (\point_i, \sphFeat_i)\}$ are formed by equipping each point $\point_i \in \Point$ with a spherical feature $\sphFeat_i \in \SphFeat$

\paragraph{Group Equivariance in CNNs} 

\haiwei{

A function $f$ is said to be equivarient to a group $\Group$ if $f(\group(x)) = (L_\group f)(x)$ for all transformations $\group \in \Group$,  where $L_{\group}$ is defined as the group operator that acts on the function $f$. 

The group convolution $$(\groupConvFunc{\group})(\point) = \int_{\group \in \Group} (L_\group f) \kernelFunc(\group^{-1}(\point))d\group$$ is equivariant to $\group$ given integrable functions $f$, $\group$ defined on $\Group$.  The translation group $\group = \mathbb{R}^3$ and the rotation group $\group = SO(3)$ are of special interests to the study of 3D shape analysis. Point convolution in 3D of the form \ref{pcconv}, naturally extending from the familiar discrete convolution, is translation-invariant (given that $h(g(x)) = (L_g h)(x)$). We thus focus our attention on the cases when $\group = SO(3)$ and $\group = SE(3)$.

}

\paragraph{Spherical Convolution}  

The spherical convolution defined in \cite{healy2003ffts} is given by: 

\begin{equation} \label{cont_sph_conv}
	 (\convFunc)(\point) = \int_{SO(3)} \sphFeat(\rotation \northPole)\kernelFunc(\rotation^{-1}\point)d\rotation
\end{equation}

where $\northPole$ is a canonical direction (north pole). Varied from the $\sphere$ correlation defined in \cite{cohen2018spherical}, this formulation allows the output of the convolution to be defined on $\sphere$. An important characteristics in \ref{cont_sph_conv} is that rotation of the canonical north pole $\northPole$ is invariant to Z-axis, therefore imposing $\kernelFunc$ to be circularly symmetric. Specifically, in the spectral domain, the convolution of $\sphFeat$ with the symmetric kernel $\kernelFunc$ is given by a weighted multiplication with Zonal Harmonic coefficients:  \((\convFunc)^m_l = \sqrt{\frac{4\pi}{2l+1}} h^0_lf^m_l\).



==> sections/result_ablation.tex <==
\subsection{Ablation Study}
\label{sec:ablation}

==> sections/result_analysis.tex <==
\subsection{Analysis of Rotation Equivariance}
\label{sec:analysis}

\weikai{We show 

\begin{itemize}
	\item visualization of our features -- by applying the rotation transform, the features are perfectly aligned
	\item comparisons with PCA based features -- show their feature is not robust again small disturbance
	\item comparisons with rotation-invariant features, e.g. PPFNet.
	\item We show that the integral of our feature, which is rotation-invariant, is worse than our rotation-equivariant features, which proves that rotation-equivariant feature is more expressive.
	\item we show we achieve better performance with even less parameters -- list a table comparing number of parameters of different networks.
\end{itemize}	
}

==> sections/result_imp.tex <==
\subsection{Experimental Setup}
\label{sec:imp}

\noindent \textbf{Datasets and Evaluation Metrics.} We conduct experiments on real-world scanning dataset 3DMatch\cite{zeng20163dmatch}, which contains eight sets of indoor scenes that are split into partially overlapped fragments. We use the 5,000 feature points provided by the authors to compute the spherical features. Following \cite{gojcic2019perfect} \shichen{add more}, we evaluate our features using two commonly used metrics, namely recall and precision, to fully demonstrate our contributions. \shichen{we set $\tau_1=0.1m$, $\tau_2=0.05$}

\noindent \textbf{Implementation Details} Our networks take \note{TBD} points as input and apply \note{TBD} stages of \convNameShort{} with stride convolution that downsample the points to \note{TBD} between each stage. 
Please refer to suppl. for the detailed network architecture and hyper-parameters used in \convNameShort{}. 
The sphere feature interpolation is performed using 3-NN interpolation with $\sigma=$ \note{TBD}.
We train the network using Adam optimizer with $\alpha=1\times 10^{-3}$ and $\beta_1=$ \note{TBD} for \note{TBD} iterations. 
The batch size is \note{TBD} for the network to fit in a single GTX 1080Ti GPU. We set the margin of batch hard loss as \note{TBD}.
Our code is implemented in PyTorch and will be made publicly available upon publication.

==> sections/result_quant.tex <==
\subsection{Quantitative Evaluation}
\label{sec:quant}


==> sections/result_time.tex <==
\subsection{Timings}
\label{sec:time}

==> sections/sup_experiment.tex <==
\section{Details on Experiment Setup}

\subsection{Details on ModelNet Training}

For each training object, we randomly sample 1,024 points from the input point cloud. We train our network with Adam optimizer. The learning rate is set to $0.001$ and the batch size is 16. The model is trained for 150 epochs with an exponential decay of learning rate by half for every 50 epochs. 

\subsection{Details on 3DMatch Training}

The training set of 3DMatch consists of RGB-D images in sequences from 62 indoor scenes. We denote a fused sequence of RGB-D images and its converted point cloud as a fragment of a scene. To generate training examples, we follow \cite{li2020end} to first fuse the RGB-D images into fragments. Then we convert the fragments to point clouds and select pairs that have more than 30\% overlapping region, given the ground-truth camera transformations. Therefore, each pair of the fragments comes from the same indoor scene. The point cloud patches used as input to the network are generated by gathering N=1,024 points within a support region whose radius is set to 0.4m. 

We train a Siamese network that extracts features from the source and target point clouds in parallel. Inspired by~\cite{gojcic2019perfect}, the network learns from a Batch Hard (BH) triplet loss, where negative examples are target patches ($\batch^p_i$) in a minibatch that do not correspond to the source patch ($\batch^a_i$):

\begin{align*} 
	\loss_{BH}(\batch) = \frac{1}{\batch}\sum^{\lvert\batch\rvert}_{i=1}&\text{max}(0, \lvert\lvert \sphFeat(\batch^a_i) -  \sphFeat(\batch^p_i) \rvert \rvert_2 -	 \\ 
	& \underset{{\substack{\text{j}=1\ldots\lvert\batch\rvert\\ \text{j}\neq\text{i}}}}{\text{min}}  \lvert\lvert \sphFeat(\batch^a_i) -  \sphFeat(\batch^p_j) \rvert \rvert_2 + m ),
\end{align*}

\noindent where $m$ is the margin for the triplet loss. We use a batch size of 16 for a mini-batch, which contains pairs of point cloud patches from the same pair of partially overlapped fragments. The model is trained for 30 epochs with an exponential decay of learning rate by half for every 6 epochs.  The choice of optimizer and all other hyperparameters remain consistent with the classification network. 


\subsection{Inference speed.} 

We compare our model used in the experiment to the baseline models that employ similar equivariant structures regarding the inference time. Specifically, we evaluated our 20-anchor model to align with the settings in~\cite{esteves2019equivariant,kanezaki2018rotationnet}. Among the selected baselines, \cite{esteves2019equivariant,kanezaki2018rotationnet} are multi-view image networks that are SO(3) equivariant; TFN~\cite{thomas2018tensor} is an example of ``non-separable'' SE(3) equivariant network. Our network is found to be faster than all of the baselines selected, and it is significantly faster than the SE(3) equivariant framework that is not separable.

\begin{table}[h]
\small
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Method   &  OURS-20 &  EMVN-20 & RotationNet & TFN \\ \hline
Time &   \textbf{35.4ms}   &      35.9ms   &   108.0ms  &  302.9ms            \\ \hline
\end{tabular}
\end{table}

==> sections/sup_network.tex <==


\section{Network Architecture and Parameters}

\begin{figure*}[h]
\vspace{-5mm}
 \begin{center}
  \includegraphics[width=0.8\linewidth]{SPNet2.png}
 \end{center}
 \caption{An illustration of the network architecture used in both ModelNet and 3DMatch experiments.}
 \vspace{-5mm}
 \label{fig:spconv}
\end{figure*}

% 32 32 64 64 128 128 256, fc: 256, stride: 2222

The network architecture used in both experiments is illustrated in Figure~\ref{fig:spconv}. Input points ($\Point \in \mathbb{R}^{\pointNum \times 3}$) are first lifted to features that are defined in the $\seThree$ space ($\SoFeat(\pointi,\soAncj): \mathbb{R}^3 \times \SoAncGroup \rightarrow \mathbb{R}$), by assigning rotation group to each point and setting its associated features to be constant 1s (denoting occupied space). 
Therefore, in the first layer, the network learns to differentiate different input points by the kernel correlation function (Equation 7 in the main text). The layer after the separable convolutional layers is an MLP layer with a symmetry function (average function) that aggregates features in the spatial dimension. We have introduced this layer as a function with implicit kernel formulation (see Equation 8 in the main text). Before the fully connected layers, a separate branch of unitary convolution takes the spatially pooled feature defined in $\soThree$, and outputs the attention confidence (see Section 3.3 in the main text). The output feature of the network can be further processed by a softmax layer in the classification task, or an $l_2$ normalization in the shape matching task. 

\section{More Implementation Details}
In the implementation of \seThree{} point convolution, we follow the design principles in~\cite{qi2017pointnet++} to compute a spatially hierarchical local structure of the points, by
 subsampling the input points with furthest point sampling and obtaining spatial local neighborhood by the ball searching algorithm. For the explicit point kernel function, we select a kernel size of 24 with kernel points evenly distributed inside a ball $\mathcal{B}_r^3$. The radius $r$ of grouping operator is set as $r^2 = d\sigma$, where $d$ is a parameter related to the density of the input points, $\sigma$ is a parameter used in the correlation function $\interCorrelation(y, \tilde{y})$ described in Section 3.1 in the main text. The kernel radius $r_k$ is set as $r_k = 0.7r$.

To achieve more effective rotation group convolution, inspired by~\cite{esteves2019equivariant}, we choose to sample the rotation group from an axis-aligned 3D model of regular icosahedral. Each face normal of the icosahedral provides the $\alpha$ and $\beta$ angles. We additionally sample three $\gamma$ angles for each face normal, each separated by 120 degrees. %The rotation is composited from the Euler angles following the xyz standard. 
The cardinality of the rotation set is thus $20 \times 3=60$. Thanks to the icosahedral symmetry, the set of rotation forms a rotation group $\SoAncGroup$ with closure, associativity, identity and invertibility. For band-limited filters, a 12-element subgroup is chosen, which transforms each element of $\SoAncGroup$ to its \soThree{} neighbors. 

It is thus worth noting that while we maintain a sparse representation for the spatial dimension of the point set, which takes online computation to find its local structure in the spatial dimension, the rotation group naturally possesses a closed grid-like structure. This greatly facilities the computation for the band-limited group convolution.   

  


==> sections/sup_proof.tex <==
\section{Proofs of equivariance}

In this section, we provide proofs of \seThree{} equivariance to the convolution introduced in the main text. Recall that the \seThree{} space can be factorized into the space of 3D rotation $\{R \vert R \in \soThree{}\}$ and 3D translation $\{\translation \vert \translation \in \mathbb{R}^3\}$. A convolution operator equivariant to \seThree{} must therefore satisfy: 
\begin{equation}
\begin{split}
  \forall \rotation \in \soThree, \rotation(\SphFeat \ast \kernelFunc)(\point, \soAnc) &= (\rotation\SphFeat \ast \kernelFunc)(\point, \soAnc), \\
    \forall \translation \in \mathbb{R}^3, \translation(\SphFeat \ast \kernelFunc)(\point, \soAnc) &= (\translation\SphFeat \ast \kernelFunc)(\point, \soAnc).
  \end{split}
\end{equation}
% We prove that the proposed \convNameFull{} is equivariant to: 1) group rotation; 2) point cloud translation.

\noindent \textbf{Theorem 1.} The continuous convolution operator \begin{multline}
  (\SoFeat \ast \kernelFunc)(\point, \soAnc) \\ =
  \int_{\pointi \in \mathbb{R}^{3}} \int_{\soAncj \in \soThree} \SoFeat(\pointi, \soAncj) \kernelFunc(\soAnc^{-1}(\point - \pointi), \soAncj^{-1}\soAnc)
  \label{equ:6d_conv_continuous}
\end{multline}
is equivariant w.r.t. rotation $\rotation \in \soThree{}$ and translation $\translation \in \mathbb{R}^3$

\textit{Proof.} Firstly, we prove that Eq.(\ref{equ:6d_conv_continuous}) is equivariant to 3D rotation. For convenience of notation, let $\pointi'=\rotation^{-1}\pointi$, and $\soAncj'=\rotation^{-1}\soAncj$. 

% Due to the closure propoerty of group, 
% \begin{equation}
%     \begin{split}
%     \forall \rotation \in \soThree{}, \{g \vert g \in \soThree{}\} &= \{\rotation g \vert g \in \soThree{}\}, \\
%   \forall x \in \mathbb{R}^3, \{g \vert g \in \soThree{}\} &= \{\rotation g \vert g \in \soThree{}\},
% %   \int_{\soAncj \in \soThree}\kernelFunc(\soAnc^{-1}(\point - \pointi), \soAncj^{-1}\soAnc) \\
% %   = \int_{\soAncj \in \soThree}&\kernelFunc(\soAnc^{-1}(\point - \pointi), \soAncj^{-1}\soAnc).
%     \end{split}
% \end{equation}


% By the definition of rotation group, $\{\soAncj'\}$ is a permutation of $\{\soAncj\}$.

\begin{align*}
\hspace{-1mm}&\rotation(\SoFeat \ast \kernelFuncInter)(\point, \soAnc) = (\SoFeat \ast \kernelFuncInter)(\rotation\point, \rotation\soAnc) \\
  &= \int_{\pointi \in \mathbb{R}^{3}} \int_{\soAncj \in \soThree} \\
    &\hspace{17mm} \SoFeat(\pointi, \soAncj)  \kernelFunc((\rotation\soAnc)^{-1}(\rotation\point - \pointi), \soAncj^{-1}\rotation\soAnc) \\
    &= \int_{\pointi \in \mathbb{R}^{3}} \int_{\soAncj \in \soThree} \\
    &\hspace{17mm}\SoFeat(\pointi, \soAncj) 
    \kernelFunc(\soAnc^{-1}(\point - \rotation^{-1}\pointi), (\rotation^{-1}\soAncj)^{-1}\soAnc) \\
    \vspace{2mm}
      &= \int_{\pointi' \in \mathbb{R}^{3}} \int_{\soAncj' \in \soThree}  \\
    &\hspace{17mm}\SoFeat(\rotation\pointi', \rotation\soAncj')  \kernelFunc(\soAnc^{-1}(\point - \pointi'), \soAncj'^{-1}\soAnc) \\
  &= (\rotation \SoFeat \ast \kernelFuncInter)(\point, \soAnc).
\end{align*}

Then, we prove that Eq.(\ref{equ:6d_conv_continuous}) is equivariant to 3D translation. Let $\pointi'=\translation^{-1}\pointi$. Because $\translation(x - x_i) = x - x_i $:

\begin{align*}
\hspace{-1mm}&\translation(\SoFeat \ast \kernelFuncInter)(\point, \soAnc) = (\SoFeat \ast \kernelFuncInter)(\translation\point, \soAnc) \\
  &= \int_{\pointi \in \mathbb{R}^{3}} \int_{\soAncj \in \soThree} \\
    &\hspace{17mm} \SoFeat(\pointi, \soAncj)  \kernelFunc(\soAnc^{-1}(\translation\point - \pointi), \soAncj^{-1}\soAnc) \\
    &= \int_{\pointi \in \mathbb{R}^{3}} \int_{\soAncj \in \soThree} \\
    &\hspace{17mm}\SoFeat(\pointi, \soAncj) 
    \kernelFunc(\soAnc^{-1}\translation(\point - \translation^{-1}\pointi), \soAncj^{-1}\soAnc) \\
    &= \int_{\pointi' \in \mathbb{R}^{3}} \int_{\soAncj \in \soThree} \\
    &\hspace{17mm}\SoFeat(\translation\pointi', \soAncj) 
    \kernelFunc(\soAnc^{-1}(\point - \pointi'), \soAncj^{-1}\soAnc) \\
  &= (\translation \SoFeat \ast \kernelFuncInter)(\point, \soAnc).
\end{align*}

The continuous convolution operator is therefore \seThree{} equivariant.
Given a finite point set $\Point$ and a finite rotation group $\SoAncGroup$, the \seThree{} separable convolution consists of two discrete convolution operators: 
\begin{align}
    (\SoFeat \ast \kernelFuncInter)(\point, \soAnc) &= \sum_{\pointi \in \Point} \SoFeat(\pointi) \kernelFuncInter(\soAnc^{-1}(\point - \pointi), \soAnc)
    \label{equ:separate_inter} \\
    (\SoFeat \ast \kernelFuncIntra)(\point, \soAnc) &= \sum_{\soAncj \in \SoAncGroup} \SoFeat(\soAncj) \kernelFuncIntra(\point, \soAncj^{-1}\soAnc)
  \label{equ:separate_intra}
\end{align}

For convenience, we use an equivalent definition in the following proof:
\begin{align}
    (\SoFeat \ast \kernelFuncInter)(\point, \soAnc) &= \sum_{\pointi \in \Point} \SoFeat(\pointi, \soAnc) \kernelFuncInter(\soAnc^{-1}(\point - \pointi))
    \label{equ:separate_inter} \\
    (\SoFeat \ast \kernelFuncIntra)(\point, \soAnc) &= \sum_{\soAncj \in \SoAncGroup} \SoFeat(\point, \soAncj) \kernelFuncIntra(\soAncj^{-1}\soAnc)
  \label{equ:separate_intra}
\end{align}


\noindent \textbf{Theorem 2.} The discrete convolution operators given in Eq.(\ref{equ:separate_inter}),(\ref{equ:separate_intra}) are equivariant w.r.t. rotation $\rotation \in \SoAncGroup$ and translation $\translation \in \mathbb{R}^3$

Again, we first prove that the two operators are equivariant to 3D rotations in the rotation group $\SoAncGroup$. Following the notations used in the previous proof, let $\Point_\rotation = \{\pointi' \vert \pointi' = \rotation \point , \point \in \Point  \}$, $G_\rotation = \{ g_j' \vert g_j' = \rotation^{-1} g, g \in G \}$:
% $\soAnc' = \rotation \soAnc$ $\SoAncGroup_\rotation = \{\rotation\soAnc \vert \soAnc \in \SoAncGroup\}$. Due to the closure property of group, $\forall \rotation \in \SoAncGroup, \soAnc' = \rotation\soAnc \in \SoAncGroup$:

\vspace{-5mm}
\begin{align*}
&\rotation(\SoFeat \ast \kernelFuncInter)(\point, \soAnc) = (\SoFeat \ast \kernelFuncInter)(\rotation\point, \rotation\soAnc) \\ &= \sum_{\pointi \in \Point} \SoFeat(\pointi, \rotation\soAnc) \kernelFuncInter((\rotation\soAnc)^{-1}(\rotation\point - \pointi))
\\ &= \sum_{\pointi \in \Point} \SoFeat(\pointi, \rotation\soAnc) \kernelFuncInter(\soAnc^{-1}(\point - \rotation^{-1}\pointi))
\\ &= \sum_{\pointi' \in \Point_\rotation} \SoFeat(\rotation \pointi', \rotation\soAnc) \kernelFuncInter(\soAnc^{-1}(\point - \pointi')) \\
&= (\rotation \SoFeat \ast \kernelFuncInter)(\point, \soAnc).
\\
\\
&\rotation(\SoFeat \ast \kernelFuncIntra)(\point, \soAnc) = (\SoFeat \ast \kernelFuncIntra)(\rotation\point, \rotation\soAnc) \\ &= \sum_{\soAncj \in \SoAncGroup} \SoFeat(\rotation\point, \soAncj) \kernelFuncIntra( \soAncj^{-1}\rotation\soAnc)
\\ &= \sum_{\soAncj' \in \SoAncGroup_\rotation} \SoFeat(\rotation\point, \rotation \soAncj') \kernelFuncIntra( \soAncj'^{-1}\soAnc)
\\
&=( \rotation \SoFeat \ast \kernelFuncIntra)(\point, \soAnc).
\end{align*}

We then prove that the two operators are equivariant to 3D translation. Let $\pointi' = \translation^{-1} \pointi$:
\vspace{-1mm}
\begin{align*}
&\translation(\SoFeat \ast \kernelFuncInter)(\point, \soAnc) = (\SoFeat \ast \kernelFuncInter)(\translation\point, \soAnc) \\ 
&= \sum_{\pointi \in \Point} \SoFeat(\pointi, \soAnc) \kernelFuncInter(\soAnc^{-1}(\translation\point - \pointi))
\\&= \sum_{\pointi \in \Point} \SoFeat(\pointi, \soAnc) \kernelFuncInter(\soAnc^{-1}\translation(\point - \translation^{-1}\pointi))
\\ &= \sum_{\pointi \in \Point} \SoFeat(\pointi, \soAnc) \kernelFuncInter(\soAnc^{-1}(\point - \translation^{-1} \pointi)) \\ &= \sum_{\pointi' \in \translation^{-1}\Point} \SoFeat(\translation \pointi', \soAnc) \kernelFuncInter(\soAnc^{-1}(\point - \pointi')) \\
&= (\translation \SoFeat \ast \kernelFuncInter)(\point, \soAnc).
\\
\\
&\translation(\SoFeat \ast \kernelFuncIntra)(\translation\point, \soAnc) = (\SoFeat \ast \kernelFuncIntra)(\translation\point, \soAnc) \\ &= \sum_{\soAncj \in \SoAncGroup} \SoFeat(\translation\point, \soAncj) \kernelFuncIntra( \soAncj^{-1}\soAnc)
\\
&=( \translation \SoFeat \ast \kernelFuncIntra)(\point, \soAnc).
\end{align*}


Since both operators are \soThree{} equivariant and translation equivariant, we have:
\begin{align*}
  \rotation((\SoFeat \ast \kernelFuncInter) \ast \kernelFuncIntra)(\point, \soAnc) &= (\rotation(\SoFeat \ast \kernelFuncInter) \ast \kernelFuncIntra)(\point, \soAnc) \\
  &= ((\rotation\SoFeat \ast \kernelFuncInter) \ast \kernelFuncIntra)(\point, \soAnc),
\end{align*}
\vspace{-5mm}
\begin{align*}
  \translation((\SoFeat \ast \kernelFuncInter) \ast \kernelFuncIntra)(\point, \soAnc) &= (\translation(\SoFeat \ast \kernelFuncInter) \ast \kernelFuncIntra)(\point, \soAnc) \\
  &= ((\translation\SoFeat \ast \kernelFuncInter) \ast \kernelFuncIntra)(\point, \soAnc).
\end{align*}

Thus, the \seThree{} separable convolution is equivariant w.r.t. rotation $\rotation \in G$ and translation $\translation \in \mathbb{R}^3$, which approximates equivariance to \seThree{}.

%\section{Feature Visualization by Choice of Global Pooling Methods}
%
%Include the figures here


==> tables/tab_3dm_ablation.tex <==
\begin{table}[]
%\small
%\addtolength{\tabcolsep}{4pt}
\caption{Average recalls under different alignment settings
} 
\centering
\begin{tabular}{c|c}
%\hline
%Methods &  Mean pool & Max pool & Unsup. atten. & Point conv & Full    \\ \hline
%Accuracy & ? & 87.4 & ? & ? & \textbf{88.3}\\ \hline
%\end{tabular}
\hline
setting &  average recall (\%)   \\ \hline
standard & \textbf{96.6}\\ 
dense & 96.5 \\ 
rotated & - \\ 
aligned & - \\ 
\end{tabular}


\label{tab:3dm_abl}
%\vspace{-7 pt}
\end{table}
